Data-Efficient 3D Visual Grounding via Order-Aware Referring

3D visual grounding aims to identify the target object within a 3D point cloud scene referred to by a natural language description. Previous works usually require significant data relating to point color and their descriptions to exploit the corresponding complicated verbo-visual relations. In our work, we introduce Vigor, a novel Data-Efficient 3D Visual Grounding framework via Order-aware Referring. Vigor leverages LLM to produce a desirable referential order from the input description for 3D visual grounding. With the proposed stacked object-referring blocks, the predicted anchor objects in the above order allow one to locate the target object progressively without supervision on the identities of anchor objects or exact relations between anchor/target objects. In addition, we present an order-aware warm-up training strategy, which augments referential orders for pre-training the visual grounding framework. This allows us to better capture the complex verbo-visual relations and benefit the desirable data-efficient learning scheme. Experimental results on the NR3D and ScanRefer datasets demonstrate our superiority in low-resource scenarios. In particular, Vigor surpasses current state-of-the-art frameworks by 9.3% and 7.6% grounding accuracy under 1% data and 10% data settings on the NR3D dataset, respectively. Our code is publicly available at https://github.com/tony10101105/Vigor.

==> figures/order_length_ablation.tex <==
\begin{figure}[t!]
  \centering
  \begin{subfigure}{0.45\linewidth}
    \includegraphics[width=\textwidth]{figures/images/order_length_performance.pdf}
    \caption{\textbf{Grounding accuracy with different maximum (padded) referential order length $B$.} Note that $B$ is equal to and denoted as the number of Object-Referring blocks.}
    \label{fig:order length performance}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.45\linewidth}
    \includegraphics[width=\textwidth]{figures/images/order_length_statistics.pdf}
    \caption{\textbf{Statistics of the referential order length in NR3D.} A longer referential order denotes a more complex referring process for grounding.}
    \label{fig:order length statistics}
  \end{subfigure}
  \caption{\textbf{(a) Grounding accuracies with varying Object-Referring block numbers $B$ and (b) statistics of referential order length of NR3D.} It can be seen that the model performance saturates at $B$=4, matching length statistics of NR3D.}
  \label{fig:order length ablation}
\end{figure}

==> tables/proposed_losses_ablations.tex <==
\begin{table}[tb]
  \caption{Ablation studies of proposed losses that help DorA better learn the concepts of anchor objects and referential order.}
  \label{tab:proposed losses ablations}
  \centering
  \addtolength{\tabcolsep}{8pt}
  \begin{tabular}{@{}ccc|cc@{}}
    \toprule
    $\mathcal{L}_{coor}$ & $\mathcal{L}_{anchor}$ & $\mathcal{L}_{mask}$ & 1\% & 100\% \\
    \midrule
     &  &  & 31.1 & 54.2 \\
     & & \ding{51} & 33.5 & 59.3 \\
     & \ding{51} & \ding{51} & 33.1 & 59.8 \\
    \ding{51} & \ding{51} & \ding{51} & 33.5 & 59.7 \\
  \bottomrule
  \end{tabular}
\end{table}
